FB-BEV: BEV Representation from Forward-Backward View Transformations

View Transformation Module (VTM), where transformations happen between multi-view image features and Bird-Eye-View (BEV) representation, is a crucial step in camera-based BEV perception systems. Currently, the two most prominent VTM paradigms are forward projection and backward projection. Forward projection, represented by Lift-Splat-Shoot, leads to sparsely projected BEV features without post-processing. Backward projection, with BEVFormer being an example, tends to generate false-positive BEV features from incorrect projections due to the lack of utilization on depth. To address the above limitations, we propose a novel forward-backward view transformation module. Our approach compensates for the deficiencies in both existing methods, allowing them to enhance each other to obtain higher quality BEV representations mutually. We instantiate the proposed module with FB-BEV, which achieves a new state-of-the-art result of 62.4% NDS on the nuScenes test set. Code and models are available at https://github.com/NVlabs/FB-BEV.

==> tables/abl_fps.tex <==
\begin{table}[htb]
\centering
\caption{Based on our experiments, we observe that FB-BEV yields slightly lower inference performance compared to BEVDet. However, we note that FB-BEV exhibits faster processing times than BEVDepth due to our model scale is much smaller than BEVDepth. The FPS is measured on RTX 3090 GPU. }
\label{tab:abl_fps}
\vspace{-1mm}
\renewcommand\arraystretch{0.7}
%\setlength{\tabcolsep}{0.6mm}
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{l|c|c|c|c|c} 
% \begin{tabular}{ p{25mm}<{\centering}| p{10mm}<{\centering} | p{12mm}<{\centering}  p{10mm}<{\centering}  p{10mm}<{\centering} p{10mm}<{\centering} p{10mm}<{\centering} p{12mm}<{\centering} | p{10mm}<{\centering}}

\toprule


\textbf{Methods} & \textbf{Temporal} & \textbf{Depth Sup.}  & \textbf{mAP}$\uparrow$  &\textbf{NDS}$\uparrow$  & FPS\\
\midrule

BEVDet  &\xmark & \xmark &0.307 & 0.382 & 19.1\\
FB-BEV & \xmark & \xmark & 0.312 & 0.406 & 16.1\\
\midrule
BEVDepth &\cmark & \cmark  & 0.370 & 0.484&13.6 \\
FB-BEV & \cmark & \cmark & 0.378&0.498& 15.3 \\


\bottomrule
\end{tabular}
}
\vspace{-1mm}
\end{table}

==> tables/abl_frpn.tex <==
\begin{table}[htb]
\centering
\caption{We show the IoU of the predicted foreground mask from FRPN.}
\label{tab:abl_frpn}
\vspace{-1mm}
\renewcommand\arraystretch{0.7}
%\setlength{\tabcolsep}{0.6mm}
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{l|c|c|c|c} 
% \begin{tabular}{ p{25mm}<{\centering}| p{10mm}<{\centering} | p{12mm}<{\centering}  p{10mm}<{\centering}  p{10mm}<{\centering} p{10mm}<{\centering} p{10mm}<{\centering} p{12mm}<{\centering} | p{10mm}<{\centering}}

\toprule


\textbf{Methods} & \textbf{Temporal} & \textbf{Depth Sup.}  & \textbf{mAP}$\uparrow$  &\textbf{NDS}$\uparrow$ \\
\midrule


FB-BEV & \xmark & \xmark & 0.312 & 0.406\\
FB-BEV & \cmark & \xmark & 0.350 & 0.479\\
FB-BEV & \cmark & \cmark & 0.378&0.498\\


\bottomrule
\end{tabular}
}
% \vspace{-1mm}
\end{table}

==> tables/abl_ft.tex <==
\begin{table}[htb]
\centering
\caption{We show the effect of adopting different foreground threshold $t_f$.}
\label{tab:abl_ft}
%\vspace{-5mm}
\renewcommand\arraystretch{0.7}
\setlength{\tabcolsep}{4mm}
\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{l|c|c|c|c} 
% \begin{tabular}{ p{25mm}<{\centering}| p{10mm}<{\centering} | p{12mm}<{\centering}  p{10mm}<{\centering}  p{10mm}<{\centering} p{10mm}<{\centering} p{10mm}<{\centering} p{12mm}<{\centering} | p{10mm}<{\centering}}

\toprule


\textbf{Methods}   & \textbf{mAP}$\uparrow$  &\textbf{NDS}$\uparrow$  & $t_f$ & IoU\\
\midrule

FB-BEV & 0.308 & 0.400 & 0.0&    -\\
FB-BEV & 0.312 & 0.406 & 0.3&    31.2\\
FB-BEV & 0.312 & 0.406 & 0.4&    49.5\\
FB-BEV & 0.312 & 0.406 &  0.5&  49.3\\


\bottomrule
\end{tabular}
}
\vspace{-1mm}
\end{table}

==> tables/abl_fusion.tex <==
\begin{table}[t]
\centering
\caption{Ablation Fusion.}
\label{tab:abl}

\resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{1pt}
\begin{tabular}{l|c|c|c|c} 
% \begin{tabular}{ p{25mm}<{\centering}| p{10mm}<{\centering} | p{12mm}<{\centering}  p{10mm}<{\centering}  p{10mm}<{\centering} p{10mm}<{\centering} p{10mm}<{\centering} p{12mm}<{\centering} | p{10mm}<{\centering}}

\toprule


\textbf{Methods} & \textbf{BEV size}   & \textbf{mAP}$\uparrow$  &\textbf{NDS}$\uparrow$  & Latency\\
\midrule

BEVDet  &128$\!\times\!$128 &0.318 & 0.410 \\
BEVDet  &256$\!\times\!$256 &0.318 & 0.410 \\
BEVDet  &400$\!\times\!$400 &0.318 & 0.410 \\

\bottomrule
\end{tabular}}
\end{table}
